AoI-based Scheduling of Correlated Sources for Timely Inference

We investigate a real-time remote inference system where multiple correlated sources transmit observations over a communication channel to a receiver. The receiver utilizes these observations to infer multiple time-varying targets. Due to limited communication resources, the delivered observations may not be fresh. To quantify data freshness, we employ the Age of Information (AoI) metric. To minimize the inference error, we aim to design a signal-agnostic scheduling policy that leverages AoI without requiring knowledge of the actual target values or the source observations. This scheduling problem is a restless multi-armed bandit (RMAB) problem with a non-separable penalty function. Unlike traditional RMABs, the correlation among sources introduces a unique challenge: the penalty function of each source depends on the AoI of other correlated sources, preventing the problem from decomposing into multiple independent Markov Decision Processes (MDPs), a key step in applying traditional RMAB solutions. To address this, we propose a novel approach that approximates the penalty function for each source and establishes an analytical bound on the approximation error. We then develop scheduling policies for two scenarios: (i) full knowledge of the penalty functions and (ii) no knowledge of the penalty functions. For the case of known penalty functions, we present an upper bound on the optimality gap that highlights the impact of the correlation parameter and the system size. For the case of unknown penalty functions and signal distributions, we develop an online learning approach that utilizes bandit feedback to learn an online Maximum Gain First policy. Simulation results demonstrate the effectiveness of our proposed policies in minimizing inference error and achieving scalability in the number of sources.

==> Evaluation.tex <==
\section{Numerical Results}
\subsection{Model-based Evaluation}
In this section, we show how to measure lower bound and upper bound by using a
\emph{Linear Time-invariant} (LTI) System. Let observation of $m$-th source $X_{m, t}$ and the target $Y_{m,t}$ evolve as follows:
\begin{align}
    X_{m, t}&=a_m X_{m, t-1}+W_{m, t},\\
    Y_{m, t}&=b_m X_{m, t}+Z_{m, t},
\end{align}
where $Z_{m, t}$ is an i.i.d. normal random variable across time, i.e., $Z_{m,t} \sim \mathcal N(0, p_m)$, the noise vector $$\mathbf W_t=\bigg[W_{1,t}, W_{2,t}, \ldots, W_{M,t}\bigg]$$ is an i.i.d. multi-variate normal random variable across time, i.e., $\mathbf W_t \sim \mathcal N(0, Q)$ and $Q$ is the covariance matrix. Let $q_{i,j}$ denote the $(i,j)$-th element of the covariance matrix $Q$. 

For this example, if $L(y, \hat y)=(y-\hat y)^2$ is a quadratic loss, then we have 

\begin{align}
\!\!  f_{\text{upper}}(\Delta_{M}(t))=
  \begin{cases}
       q_{m,m} b_m^2 \Delta_{M}(t)+p_m, &\text{if}~a_m=1,\\
       q_{m,m} b_m^2 \frac{a_m^{2\Delta_{M}(t)}-1}{a_m^2-1}+p_m, &\text{otherwise.}\\
    \end{cases}
    \end{align} 

\begin{align}
\!\!  f_{\text{lower}}(\Delta_{M}(t))=
  \begin{cases}
       \bar q_{m,m} b_m^2 \Delta_{M}(t)+p_m, &\text{if}~a_m=1,\\
       \bar q_{m,m} b_m^2 \frac{a_m^{2\Delta_{M}(t)}-1}{a_m^2-1}+p_m, &\text{otherwise,}\\
    \end{cases}
    \end{align} 
    where $\bar q_{m,m}=q_{m,m}-\mathbf q_m Q^{-1}_{-1} \mathbf q_m^T$, $\mathbf q_m=[q_{m,1}, \ldots, q_{m,m-1}, q_{m, m+1}, \ldots, q_{m, M}]$ is the covariance of the $m$-th noise process with other process, and $Q^{-1}_{-1}$ is the noise covariance sub-matrix of the other processes.

\subsection{Data-driven Evaluation}
    

==> InformationTheory.tex <==
\section{Information-theoretic Analysis of Inference Error}

In this section, we present an information-theoretic analysis of the inference error $\mathbb E_{\pi}[L(Y_{m, t}, \hat Y_{m,t})]$ by establishing both an upper and a lower bound. This information-theoretic analysis facilitates a  tractable design of scheduling policy. 

Specifically, we will use $L$-information-theoretic metrics studied in \cite{dawid1998, farnia2016minimax, shishertimely}. The $L$-entropy of a random variable $Y$ is defined as \cite{dawid1998, farnia2016minimax, shishertimely}: 
\begin{align} \label{gen_def_L_entropy}
H_L (Y) = \min _{y \in \mathcal{Y}} \mathbb{E}_{Y \sim P_Y} [L (Y, y)].
%H_L (Y_{n,t}) = \min _{a \in \mathcal{A}} \mathbb{E} [L (Y_{n,t}, a)].
\end{align}
The $L$-conditional entropy of $Y$ given $X=x$ is given by  \cite{dawid1998, farnia2016minimax, shishertimely}:
\begin{align} \label{L_cond_enx}
H_L (Y | X=x)
=\min _{y \in \mathcal{Y}} \mathbb{E}[L (Y, y)|X=x],
\end{align} 
and the $L$-conditional entropy of $Y$ given $X$ is
\begin{align} 
\label{L_cond_en}
H_L (Y | X)
=\mathbb{E}[H_L (Y | X=x)].
\end{align} 

\begin{theorem}\label{theorem1}
The following assertions are true:
\begin{itemize}
\item[(a)] The inference error for target $Y_{m,t}$ can be expressed as
\begin{align}
    &\mathbb{E}\left[L(Y_{m,t}, \hat Y_{m,t})\right]\nonumber\\
    &=H_L\bigg(Y_{m,t}|(X_{m, t-\Delta_{m}(t)}, \Delta_{m}(t))_{m=1}^M\bigg),
\end{align}
where $\Delta_{m}(t)$ is the AoI of source $m$ under the scheduling policy $\pi$.
\item[(b)] An upper bound of the inference error for target $Y_{m,t}$ is given by  
        
\begin{align}
&\mathbb{E}\left[L(Y_{m,t}, \hat Y_{m,t})\right]\nonumber\\
&\leq H_L\left(Y_{m,t}|X_{m,t-\Delta_{m}(t)}, \Delta_{m}(t)\right)   
\end{align}

\item[(c)] If the targets and the signal observations satisfy the following Markov chain
$$(i)  Y_{m, t} \leftrightarrow X_{m', t-1} \leftrightarrow X_{m', t-\mu},$$ then a lower bound of the inference error for target $Y_{m,t}$ is given by  
        
\begin{align}
&\mathbb{E}\left[L(Y_{m,t}, \hat Y_{m,t})\right] \nonumber\\
&\geq H_L\left(Y_{m,t}|X_{m,t-\Delta_{m}(t)}, \Delta_{m}(t), \mathbf X_{-m, t-1}\right).   
\end{align}.
\end{itemize}
\end{theorem}
\begin{proof}
    See Appendix.. 
\end{proof}
Theorem \ref{theorem1}(a) states that the inference error for target $Y_{m,t}$ can be expressed as a $L$-conditional entropy of the target $Y_{m,t}$ given the latest received signal observations $$(X_{1, t-\Delta_{1}(t)}, X_{2, t-\Delta_{2}(t)}, \ldots, X_{M, t-\Delta_{M}(t)})$$ and their AoI values $$(\Delta_{1}(t), \Delta_2(t), \ldots, \Delta_M(t)).$$ 

Theorem \ref{theorem1}(b) provides an information-theoretic upper bound on the inference error. When considering information solely from source $m$, the inference error for the $m$-th target is given by
$$H_L\left(Y_{m,t}|X_{m,t-\Delta_{m}(t)}, \Delta_{m}(t)\right).$$
Since this excludes information from other sources, the resulting inference error is higher than the actual inference error achievable when incorporating information from all sources. In the specific scenario where the target $Y_{m,t}$ is uncorrelated with the information from other sources, this upper bound coincides with the actual inference error.

Theorem \ref{theorem1}(c) establishes an information-theoretic lower bound on the inference error. This lower bound, given by
$$H_L\left(Y_{m,t}|X_{m,t-\Delta_{m}(t)}, \Delta_{m}(t), \mathbf X_{-m, t-1}\right),$$
represents the inference error that would arise if updates were received from all sources other than $m$. However, in practice, constraint \eqref{Scheduling_constraint1} may prevent scheduling all sources at every time slot. Consequently, the actual inference error is higher than this lower bound, as less information will be available for inference. The lower bound becomes equal to the actual inference error if (i) the target $Y_{m,t}$ is uncorrelated with the information from other sources or (ii) all sources other than $m$ are scheduled at time slot $t$.





%The problem \eqref{Multi-scheduling_problem1}-\eqref{Scheduling_constraint2} is a restless multi-armed bandit (RMAB) problem. Many researchers utilized Whittle index policy to solve RMAB problem. The first approach to get Whittle index policy is to decompose \eqref{Multi-scheduling_problem1}-\eqref{Scheduling_constraint2} into $M$ independent sub-problems, where each sub-problem $m$ is associated with source $m$. We can not directly get Whittle index policy because the cost function $g_m(\Delta_{1}(t), \Delta_{2}(t), \ldots, \Delta_{M}(t))$ for source $m$ depends on the AoI values of other sources. To overcome this challenge, we get a lower bound $f_{\text{lower}}(\Delta_{M}(t))$ and an upper bound $f_{\text{upper}}(\Delta_{M}(t))$ of $g_m(\Delta_{1}(t), \Delta_{2}(t), \ldots, \Delta_{M}(t))$.






